Understanding Gaps in LLM Pipelines Towards Scalable Fuzzing Harness Generation: An Empirical Study and Enhancement

Large language model (LLM)-based techniques have achieved notable progress in fuzz harness generation. However, applying them to arbitrary functions \textit{at scale} remains difficult---generated harnesses often fail to compile or, worse, compile but remain logically ineffective. What factors drive success and what limitations hinder current methods remain unclear. To answer these questions, we conduct an empirical study on state-of-the-art LLM-based harness generation frameworks across 29 OSS-Fuzz projects. Our study establishes two pillars of success: contextual information to guide generation and pre-structured pipelines that ensure workflow stability. However, significant gaps remain: (1) existing context retrieval methods lack the robustness to reliably obtain necessary information across diverse projects; (2) current validation mechanisms fail to detect logically ineffective harnesses, such as those containing fabricated definitions; and (3) compilation workflows are brittle, unable to distinguish harness-level errors from build-configuration issues. We demonstrate the utility of these findings by enhancing existing techniques with a hybrid tool pool for robust context retrieval, an enhanced validation pipeline, and a compilation-error triage strategy. Evaluated on 243 OSS-Fuzz projects (65 C and 178 C++), the enhanced approach improves the three-shot success rate by approximately 20\% over state-of-the-art techniques, reaching 87\% for C and 81\% for C++. Our one-hour fuzzing results show that more than 75\% of the generated harnesses increase target-function coverage, surpassing baselines by over 10\%. In addition, the enhanced approach identified 15 new vulnerabilities across 11 real-world projects.

==> figure/tool_call_overall.tex <==
\begin{figure}[h]
    \centering
   \includegraphics[width=\columnwidth]{figure/tool_call_groupbar.pdf}
    \vspace{-1em}
    \caption{The number of total tool calls and the number of corresponding responses with \our~tool and the Fuzz Introspector tool.}
    \label{fig:tool-overall}
\end{figure}
